VIOLA: Imitation Learning for Vision-Based Manipulation with Object Proposal Priors

We introduce VIOLA, an object-centric imitation learning approach to learning closed-loop visuomotor policies for robot manipulation. Our approach constructs object-centric representations based on general object proposals from a pre-trained vision model. VIOLA uses a transformer-based policy to reason over these representations and attend to the task-relevant visual factors for action prediction. Such object-based structural priors improve deep imitation learning algorithm's robustness against object variations and environmental perturbations. We quantitatively evaluate VIOLA in simulation and on real robots. VIOLA outperforms the state-of-the-art imitation learning methods by $45.8\%$ in success rate. It has also been deployed successfully on a physical robot to solve challenging long-horizon tasks, such as dining table arrangement and coffee making. More videos and model details can be found in supplementary material and the project website: https://ut-austin-rpl.github.io/VIOLA .

==> backup_files/03_method.tex <==
\begin{figure}[t]
    \centering
%\begin{minipage}[t]{0.9\textwidth}
% \makeatletter\def\@captype{figure}
    \includegraphics[width=1.0\linewidth, trim=0cm 0cm 0cm 0cm,clip]{figures/Model.pdf}
    \vspace{-5mm}
    \caption{Model architecture of \ourmethod{}. Given an observation at time $t$, we first compute the object-centric features $h_t$ per state using top $K$ object proposals. Then we construct the object-centric representation $z_t$ by composing $\{h_{t-i}\}_{i=0}^{H}$. After having $z_t$, we use a transformer to condition action on $z_t$ and the latent vector action (latent actions) output from the transformer is passed though a multi-layer perceptron (MLP) to compute the task-space command as the action outputs.\yuke{what constitutes a token?}}
    \label{fig:viola-approach}
    % \vspace{-4mm}
%\end{minipage}
\end{figure}


% We introduce our approach \ourmethod{} that learns policies for visuomotor manipulation using behavior cloning algorithm. The overview of \ourmethod{} is visualized in Figure~\ref{fig:viola-approach}. 

% The approach can be mainly divided into two parts: 1) Computing an object-centric representation that is spatial-temporal, and 2) computing the robot's action using a transformer-based module. Overall the two parts are trained in an end-to-end manner so that the approach is as straightforward as state-of-the-art baselines.

% \todo{Our model first take in top $K$ object proposals from the workspace image using a pretrained RPN, which proposes the regions that more likely contain objects. Then we construct a spatio-temporal form of the object-centric representation on top of features of proposals, which is described in more details later. Once we have the input representaiton, we use a transformer-based module to reason over the set of individual tokens in the representation, and computes the task-space command for manipulation.}


\subsection{Object-Centric Representation}
 Our goal is to design the object-centric representations for policies to reason over object features and compute the task-space commands. Learning the object-centric representations consists of two main steps: 1) We use a feature encoder to learn object-centric features at each time step and 2) we compose the features from a history of observations to form the object-centric representation.

\paragraph{Feature Encoder} Given an observation $s_t$ at time $t$, we compute an object-centric feature $h_t$ \yuke{[what is state???] for each state}. Specifically, we first obtain bounding boxes of top $K$ object proposals by using a pre-trained RPN on the workspace image. The intuition behind using a pre-trained RPN is that it captures good priors of ``objectness'' in RGB images by training on large image datasets. \yuke{[causal relation is weak] Therefore, we directly use a pre-trained RPN to localize objects in both our simulated and real-world tasks.} As RPNs predict the proposals along with confidence, we choose the ones with top $K$ confidence scores for every time step. 
%Furthermore, as pre-trained RPNs are agnostic to our demonstration data, we can use them to localize objects in  observations from demonstrations due to distributional shift or environment noises. 
In this work, we choose to use RPN from Zhou et al.~\cite{zhou2022detecting}, which shows promising results for detecting a wide range of everyday objects from two thousand classes.


 Once we get the top $K$ proposals,
 we \yuke{[you have used ``learn'' all over the place, not sure that's the right verb. in some places, it feels more like ``extract'' or ``build''] learn} the object-centric feature $h_t$ at each time step. The main component of $h_t$ is the object proposals that encode both their visual features and positional features.\yuke{why? remind the audience why we need these two features} We directly use the bounding box positions of proposals for positional features but learn the visual features from scratch. The reason behind this design is that our manipulation task shares the same objective of localizing objects as the vision tasks, but they differ in the downstream tasks: pre-trained models optimized the visual features for classifications but we aim to optimize them for continuous motor control. For positional features, we encode the bounding box positions through sinusoidal positional encoding. As such a positional encoding informs the relative positional information due to the use of sinusoidal functions~\cite{vaswani2017attention}, it allows policies to reason over positional relations among proposals. For the visual features, we first encode workspace images into spatial feature maps using ResNet-18 based convolutional layers and extract the features using ROI pooling~\cite{girshick2015fast}. We map the positional encodings to the same dimension as visual features so that we can add them up to obtain the proposal features, which we refer to as proposal tokens later.\yuke{writing style comments: reduce the use of ``and ... then'', ``first'', ``directly'', ``actually''. in most cases, they can be deleted}
 
 % For the visual features, we first encode  workspace images into spatial feature maps using ResNet-18 based convolutional layers and extract the features using ROI pooling~\cite{girshick2015fast}. We extract visual features from the spatial feature map instead of directly using pre-trained models because visual features from pre-trained models are optimized for downstream vision tasks such as classification, while we need the visual features of object proposals that are otpimized for visuomotor control task. For positional features, we use the proposals' bounding box positions to encode the information of locations and sizes of the objects. We encode the bounding box positions through sinusoidal positional encoding. As such a positional encoding informs the relative positional information based on sinusoidal functions~\cite{vaswani2017attention}, it allows reasoning over positional relations among proposals. We map the positional encodings to the same dimension as visual features so that we can add them up to obtain the proposal features, which we refer to as proposal tokens later.
  
 % \yuke{[broken sentence and how you learn the new visual features?] We learn new visual features instead of directly using a pre-trained model is that the visual features from pre-trained models are optimized for downstream vision tasks such as classification, while we need the visual features that are optimized for visuomotor control tasks.} For \yuke{[I think we should change a name to this. the visual feature is also spatial. we need a more descriptive name] spatial features}, we use the proposals' bounding box positions to encode information of locations and sizes of the objects. We encode the bounding box positions \yuke{[confusing how sinusoidal positional encoding allows reasoning?] through sinusoidal positional encoding to allow reasoning over spatial features~\cite{vaswani2017attention}.} \yuke{[you used a lot of And at the start of sentences. in 99\% of the time, they can be removed] And we} map positional encodings to the same dimension as visual features so that we can add them up to obtain the proposal features.
 
 While we get a factorized representation based on object proposals, two additional challenges remain: 1) \yuke{[still not sure what this sentence means] individual object proposals lack the information about the current stage of the task}, and 2) a robot's end-effector may block the camera view and occlude some objects. To tackle the first challenge, we need features that inform policies about the context of the current task stage. Such \yuke{[information is uncountable] a information} is most straighforward to infer from the workspace image, and we compute the context feature by projecting the spatial feature map into a latent vector, which we refer to as a global context token. 
 %To achieve this, we project the spatial feature map computed from the workspace image into a global context token to provide \yuke{[you used the context a lot of times, but it was still unclear to me what this means exactly. is it just the background objects or something else? and how it informs the task progress?] the context of task progress}; 
 To address the second challenge, we include a feature token that is computed from eye-in-hand camera to mitigate occlusion. Along with these tokens, we also include tokens that are mapped from the robot's proprioceptive information. We refer to all these tokens as \yuke{[use a more descriptive name] context features}, which are concatenated with proposal features to build the object-centric features $h_t$ at each time step.

% All these tokens are computed as in the same size as the object tokens. More concretely, we compute a latent vector, context token, computed from the spatial feature map. A eye-in-hand token is computed from an eye-in-hand image. Proprioception tokens are computed through linear projection from the states of arms and grippers individually. For these states, we use the joint states and the gripper states as they are the two observations that are directly available from perception.

\paragraph{Temporal composition} We consider object-centric features from a history of observations to model the temporal correlations among observations. The temporal modeling has shown beneficial in imitating from human demonstrations as human make decisions depending on history information~\cite{mandlekar2020iris, mandlekar2021matters}.\yuke{need intuition! why this would be better. saying that it has better results in prior work is not enough} Therefore, we build our object-centric representation through temporal compositions of object-centric features $h_t$. Temporal composition also directly brings the benefits of increasing the recall coverage of object proposals over objects as RPNs would inevitably miss detecting objects at some frames. 

Concretely, we aggregate object-centric features $\{h_{t-i}\}_{i=0}^{H}$ of the last $H+1$ time steps to build the object-centric representation $z_t$. As we mention before, we use a transformer in our policy,  which is permutation-invariant to input ordering. To retain the temporal information in the input sequence, we add sinusoidal positional encoding of temporal positions in a sequence~\cite{vaswani2017attention}, $\{PE_{i}\}_{i=0}^{H}$, to object-centric features $h_{t}$. Eventually, we \yuke{[no ``can'', either you did it or you didn't] can} get the object-centric representation $z_t = Concat(\{h_{t-i}\oplus PE_{i}\}_{i=0}^{H})$. As our ablation experiment in the later section suggests, the use of temporal positional encoding enables the modeling of temporal correlations from demonstrations, giving better performance than policies without temporal information.

\subsection{Transformer-based Policy}
Our goal is to design a policy that attends more to task-relevant tokens (features) in object-centric representation $z_t$ so that the task-relevant tokens dominate the action computation.  The intuition behind this goal is that the robot actions conditions on the states of task-relevant objects, and tokens associated with task-relevant proposals can help predict actions easily while tokens with task-irrelevant ones confounds predictions. We naturally seek to the transformer~\cite{vaswani2017attention} as the policy backbone, \yuke{[why self-attention can determine this?] which can determines task-relevant tokens and task-irrelevant ones through its self-attention mechanism}. The transformer takes all the tokens as inputs and compute attention masks over them to select the task-relevant tokens. By training the transformer on the demonstration data, we expect large attention weights on the task-relevant tokens, and that would allow task-relevant tokens dominate the action computation.

In practice, to compute robot actions that conditions on the tokens from $z_t$,  we introduce a learnable vector, action token, that passes through the transformer along with $z_t$. Such a design has resemblance to the specific class tokens in natural language understanding tasks~\cite{devlin2018bert} or in visual recognition tasks~\cite{dosovitskiy2020image}. \yuke{[wrong grammar] At the output of the transformer, we have a latent vector, \yuke{[is this term necessary? avoid defining new concepts unless absolutely needed] ``latent action''}, that corresponds to the action token}. We pass this latent action through a two-layered fully-connected networks, followed by a GMM (Gaussian Mixture Model) output head. We use the design of GMM output head for its effectiveness to learn from diverse demonstrations, which has been shown in related work~\cite{wang2020critic, mandlekar2021matters}.


% concatenate a learnable vector, action token with $z_t$ and pass them through the transformer. T

% and the action token is  through the transformer along with $z_t$ to output a latent action vector, and the latent action vector is pa

% and the latent action vector at the transformer's output for action computation. 

% \sketch{1. our goal is to design policy so that it can attend more to ; 2) the key is to compute attentions to weigh more on and .. .  The transformer takes in a set of tokens, and use its self-attention mechanisms to weigh more on some tokens and . For our use case, 
% our object-centric representation is factorized by tokens; 2. and }

% \sketch{1. transformer takes in a set of tokens, and reaonss over tokens to compute output}

% Our goal is to design a policy that attends more to task-relevant tokens in object-centric representation $z_t$ to compute the robots' actions.

% \paragraph{Transformer-based Module}
% \sketch{1. We want to attend more to task-relevant\\ 2. the transformer attends with different weights; \\ 3. why can it pay attention to task-relevant? Because attending more to task-relevant objects could help capture the correlation between observations and actions more easily.}
% \yuke{transformer should be mentioned in 3.1 to pave the path for describing 3.2} Our goal is designing a policy that attends more to task-relevant tokens (features) in object-centric representation $z_t$ to compute the robots' actions. \yuke{[rewrite! describe on a high-level what transformer does, and why it can be used to identify task-relevant objects] There are two major components in this process: We first need to compute over proposal tokens and context tokens to decide which proposal tokens are more relevant to tasks, then we want to compute robot commands by considering more on the task-relevant tokens. To realize these requirement, we naturally seek to a transformer architecture, which naturally weighs the input feature tokens using its self-attention mechanism. We pass $z_t$ into a transformer module which consists of multiple transformer blocks sequentially, and the policies can reason about which tokens are more relevant to tasks. }

% \paragraph{Policy Action Output} \sketch{As our input tokens are heterougenous, spanning across different modalities, which might have different scales. So we include an action token that is learnable that can take into account different modalities of data. Similar design principle is also adopted by many vision applications, such as in ViT, visualBert ... } To compute actions that condition on the feature tokens, we use an action token which is a learnable vector, that specifically take into account the attended features\yuke{why this token is needed?}. In practice, we pass the  action token into the transformer along with $z_t$, \yuke{[I don't understand this] so that the action token can take into account the attentions across different layers of transformer blocks}. The output of the transformer corresponding to the action token is a \yuke{[how is this relevant to your latent actions in fig 2] latent vector.} We pass the latent vector through a two-layered fully-connected networks, followed by a GMM (Gaussian Mixture Model) output head. We use the design of GMM output head for its effectiveness to learn from diverse demonstrations as shown in \yuke{[``related work'' is usually uncountable unless in certain context, e.g., these two related works focus on blah blah...] recent works~\cite{wang2020critic, mandlekar2021matters}}.


% \sketch{1. Once we have the object-centric representation, we want to reason over which object-centric features are most relevant, and condition the actions on it. \\ 2. Therefore, we naturally seek to transformer architecture, which naturally weighs on the input features using its self-attention mechanism. The self-attention mechanism naturally has two benefits: a) provides attention over input features; b) contextualize object features by computing the relation with context tokens in the input; 3. moreover,  the output conditions on the attention computation inside the transformer; \\ 4. For computing robot commands, we also make a action-specific designs to disentangle computation from reasoning over object-centric features: a learnable tensor, action token, which passes along with $z_t$ to obtain a latent vector $\hat{a}_{t}$, and the latent vector is passed through fully connected network to compute action $a_t$. In order to better capture the diverse behaviors in demonstration data, we choose GMM output head to further capture the multi-modality of low-level actions that exist in demonstrations.  }

% \paragraph{Transformer Reasoning}
% Once we have the spatio-temporal representation $z_{t}$ from perception, we can pass $z_{t}$ through the transformer. With the self-attention mechanism in transformers, we can obtain a soft attention over object-features that are also conditioned on all the context features in the $H+1$ temporal sequences. Without context features, the transformer is hard to determine which object features should be used for reasoning over the downstream manipulation actions. Also, as our input features into the transformer has various modality, we introduce a single learnable tensor, action token, for learning the latent vector of computing manipulation actions.

% \paragraph{Policy Action Output}

% Once we have the object-centric, spatio-temporal representations, we use a transformer-based policy to compute the action of the robot.  As we pass all tokens through the transformer module, we obtain the output of action token that can be used for computing the robot's task-space command. More concretely, we pass the action token through a 
% two-layered fully connected networks, followed by a GMM (Gaussian Mixture Model) output head. Using such a multimodal output representation 
% GMM (Gaussian Mixture Model) MLP layers. We choose GMM MLP layers as the demonstrations are often diverse, and such a probabilistic output head has shown better result in capture those diverse behavior (cite Deepmind, robomimic). 


%\subsection{Object-centric Spatial Module}Once we have the object-centric, spatio-temporal representations, we use a transformer-based 

%The first important module in \ourmethod{} is Object-centric Spatial Module (OSM). OSM is designed to to obtain per-timestep representation from raw perception. Specifically, we apply a pretrained region proposal network to get top $K$ object proposals (Cite Visual Bert). This is to approximately cover the objects that are involved in the task. Then instead of using detection labels which lack the temporal consistency for such a temporally-extended manipulation task, we instead extract visual features of the object proposals through ROI pooling operations (citation) on the spatial feature map. Then we flatten each ROI feature to get a latent vector token. Moreover, to keep the spatial information of object proposals, we compute the sinusoidal positional encoding using proposal's bounding box coordinates, and add them back to each of their extracted visual features. With such a sinusoidal positional encoding, we naturally encode positional information into the visual features, and such a periodic positional encoding naturally provides the information of spatial relations (citation). 

%\paragraph{Context features and assistive perception} Our object


%\paragraph{assistive perception}So far, the visual features we extracted are based off object proposals which are agnostic to the downstream manipulation task. While the proposals can provide a very good coverage of the objects in the scene, it contains false positive proposals and lacks the information of which objects are relevant to the current stage of the task. Therefore, we also compute context features based on the spatial visual feature map, along with other assistive observations, namely eye-in-hand images and robot's proprioception. The spatial visual feature map is processed into a latent vector of context features using spatial softmax as a strong normalization of the feature. Eye-in-hand images provide useful visual information when contacting with one object because typically the object will be occluded by the gripper in the workspace view. Therefore we use ResNet-18 followed by spatial softmax layer to obtain spatial keypoints to provide such information. The proprioception is easy to access and provide accurate information about robot's own state, which would be hard to infer visually. We just do a linear mapping on the state of arm and state of gripper to obtain two vectors with the same size as the latent features of object proposals. With the context features along with assistive features, the transformer module can unleash its self-attention mechanism to reason over which object proposals are more relevant to current stage of tasks.

% \subsection{Spatio-Temporal Transformer}


% \paragraph{Spatio-Temporal Representation} After we obtain per-timestep representations $\{h_t\}$, we design a spatio-temporal representation on top of them so that we can reason over both spatially and temporally. More concretely, at time step $t$, we consider $H+1$ consecutive OSM representation$\{h_{t-i}\}_{i=0}^{H}$ (clip at $0$ if t < $H$). As transformer is not a recurrent architecture~\cite{}, we need to inform the transformer about the temporal order of inputs. More concretely, we add a temporal positional encoding $PE_{i}$ in the form of sinusoidal functions ~\cite{} to $h_{i}$ to inform the following transformer model about temporal information of observation, and we get $\bar{h}_{i} = h_{i} \oplus PE_{i}$. After this operation, we can obtain a spatio-temporal representation $z_{t}$ which consists of all the OSM representation. Natrually such a spatio-temporal representation is object-centric as it contains all the object-centric features from OSM in $H+1$ timesteps.

% The benefits of such a spatio-temporal representation are three-folds: 1) we can naturally encode spatial information of object proposals in per-timestep representation $h_{t}$; 2) such a representation can cover objects more robustly in case there are occasional missing detections at each timestep; 3) such a representation can naturally model the hidden  variables underneath temporal sequences of demonstrations.

% \paragraph{Transformer Reasoning} 
% Once we have the spatio-temporal representation from perception, we can pass it through a spatio-temporal transformer to reason over
% Our spatio-temporal transformer takes into account xxxx. In order to keep the temporal information of observations, we provide temporal positional encoding (sinusoidal functions). 

% Given object proposals, purely knowing their spatio-temporal information is insufficient for transformer to reason better about which object proposals should pay more attention to. The key to operationalize this is the spatial visual feature map mentioned in the first subsection.


% Highlight several key designs:
% 1. Temporal one
% 2. spatial object proposal tokens
% 3. context-dependent (callback on the first subsection to explain why using workspace image token --- to rationalize task-dependent object proposals). 

==> backup_files/03_problem.tex <==
We present \ourmethod{}, an object-centric imitation learning approach to vision-based manipulation. The core idea is to factorize high-dimensional visual observations into object-centric representations, on top of which the policy computes closed-loop control actions. An overview of the \ourmethod{} model is illustrated in Figure~\ref{fig:viola-approach}. 
% \ourmethod{} first takes in top $K$ object proposals from the workspace image using a pretrained RPN, which proposes the regions that more likely contain objects. Then we construct a spatio-temporal form of the object-centric representation on top of features of proposals, which is described in more details later. Once we have the input representaiton, we use a transformer-based module to reason over the set of individual tokens in the representation, and computes the task-space command for manipulation.
Here we first formulate the problem of visuomotor policy learning. We describe the two key components of \ourmethod{}: 1) how we construct the object-centric representations based on general object proposals, and 2) how we use a transformer-based policy architecture to reason over the object-centric representations for predicting actions.

\subsection{Problem Formulation}
% We consider the problem of solving vision-based manipulation tasks under the framework of imitation learning.
We formulate a robot manipulation task as a discrete-time Markov Decision Process, which is defined as a 6-tuple: $\mathcal{M}=(\mathcal{S}, \mathcal{A}, \mathcal{P}, R, \gamma, \rho_{0})$, where $\mathcal{S}$ is the state space, $\mathcal{A}$ is the action space, $\mathcal{P}(\cdot|s, a)$ is the stochastic transition probability, $R(s, a, s')$ is the reward function, $\gamma \in [0, 1)$ is the discount factor, and $\rho_{0}(\cdot)$ is the initial state distribution. In our context, $\mathcal{S}$ is the space of the robot's raw sensory data, including RGB images and proprioception, $\mathcal{A}$ is the space of the robot's motor commands, and $\pi: \mathcal{S}\rightarrow\mathcal{A}$ is a closed-loop sensorimotor policy that we deploy on the robot to perform a task. Our goal is to learn the policy $\pi$ from a set of human demonstrations that maximizes the expected return $\mathbb{E}[\sum^\infty_{t=0}\gamma^t R(s_t, a_t, s_{t+1})]$.

\yuke{As objects are the basic constituents of manipulation scenes, we factorize the state space of such MDP based on objects.} For a manipulation task, there exists a set of objects that we can use to represent the state space based on $\mathcal{O}=\{o_1, o_2, \dots, o_N\}$. In unstructured environments, ground-truth physical states of objects are inaccessible to the robot. Instead, at each time $t$, we generate $K$ object proposals  $\mathcal{\bar{O}}(t)=\{\bar{o}_{1}(t), \bar{o}_{2}(t), \dots, \bar{o}_{K}(t)\}$ from a pre-trained Region Proposal Network~\cite{ren2015faster} at time $t$, where $\bar{o}_{k}(t)$ is an object proposal on 2D images that consists of the bounding box position and the visual feature inside bounding box. We denote the feature of a proposal $\bar{o}_{k}(t)$ as $f(\bar{o}_{k}(t))\in \mathbb{R}^{D}$ that is based on its visual feature and the bounding box position, and $D$ is the feature dimension.

In our work, we consider an object-centric representation $z_t$ that is based on object proposals from observations of the last $H+1$ time steps to model the temporal correlations between observations. Concretely, we aggregate features of $K$ object proposals $\{f(\bar{o}_{k}(t))\}_{k=1}^{K} \in \mathbb{R}^{K\times D}$ along with \yuke{[what does "contextualize the proposals" mean?] $M$ features $\{f_{m}\}_{m=0}^{M}\in \mathbb{R}^{M\times D}$ that are learned from images and proprioception to contextualize the proposals}. These features are stacked together into $h_{t}\in \mathbb{R}^{(K+M)\times D}$, which we refer to as object-centric features at time $t$. Then we build an \yuke{[confusing between object-centric representation and object-centric feature] object-centric representation} $z_t \in  \mathbb{R}^{(H+1)(K+M)\times D}$ by concatenating the $h_t$ in the past $H+1$ time steps. Our policies that condition on object-centric representations can be written as $a\sim \pi(\cdot|z)$. We refer to each $1\times D$ row vector in $z_t$ as a \textit{token}. Our policy uses a transformer\yuke{cite} as the model backbone that takes in a sequence of tokens and outputs the same number of $1\times D$ latent vectors through its self-attention architecture\yuke{refer to 3.3}. 

% \todo{Describe transformers how to process tokens}For reasoning over $z_t$, we use a transformer-based policy. Transformer is a recent deep-learning architecture that uses self-attention mechanisms to process a list of input features. In the context of transformers, tokens are ... . Transformer takes in a number of input tokens, and compute latent vectors for all the tokens. 

% \yuke{Define the object proposals as bounding boxes + features.} We use features from $K$ object proposals $\mathcal{\bar{O}}=\{\bar{o}_{1}, \bar{o}_{2}, \dots, \bar{o}_{K}\}$ as \yuke{formalize what is ``object-centric representation'' before starting referring to it} the object-centric features in our object-centric representation. We denote our \yuke{[what's the relationship between $z_t$ and $\bar{O}$?] object-centric representation $z_t$} at time $t$. So our policies that condition on object-centric representation can be written as $a\sim \pi(\cdot|z)$.

% \begin{align*}
%     \psi&: \mathcal{S} \mapsto \mathcal{Z} \\
%     \pi&: \mathcal{Z} \mapsto \mathcal{A} \\
% \end{align*}
% Where $\psi$ is the representation learning module, and $\pi$ is the policy that conditions on the object-centric representation to compute robot actions.

==> backup_files/backup_evaluation.tex <==
Base (Transformer) & 69.5 $\pm$ 2.5 & 25.1 $\pm$ 2.2 & 37.7 $\pm$ 3.4 & 39.9 $\pm$ 1.5 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 &\\
+ Temporal position & 74.0 $\pm$ 0.8 & 48.3 $\pm$ 1.9 & 48.3 $\pm$ 3.3 & 50.9 $\pm$ 1.5 & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & 0.3 $\pm$ 0.2 & 0.0 $\pm$ 0.0\\
+ Object proposals & 72.8 $\pm$ 0.9 & 37.7 $\pm$ 1.2 & 54.6 $\pm$ 4.6 & 49.2 $\pm$ 1.6  & 49.8 $\pm$ 2.5 & 19.1 $\pm$ 0.7 & 28.4 $\pm$ 3.6 & 25.7 $\pm$ 0.6\\
+ Proposal locations & 80.2 $\pm$ 2.9 & 38.6 $\pm$ 0.3 & 62.0 $\pm$ 5.7 & 46.5 $\pm$ 1.9 & 80.2 $\pm$ 3.0 & 36.9 $\pm$ 1.0 & 48.2 $\pm$ 6.1 & 34.0 $\pm$ 0.8\\

==> backup_files/intro_note.tex <==
\subsection{Motvation}
1. Goal: imitation learning on general object-centric representations for manipulation policies
2. Why imitation learning
3. Why is it hard?
4. We learn robust and generalizable policies by learning object-centric imitation policies.

We also need to explain several things:
1. Why not use object states directly(it is hard to get 3D CAD models of objects in the wild). We need the inductive bias of "objectness", but without assuming ground-truth access. For a specific manipulation tasks, the perception of "objects" is task dependent.

\begin{itemize}
    \item Real-world manipulation tasks are challenging.
    \item Imitation learning has been a data-efficient paradigm for robots to learn a manipulation policy without hand-designing motor programs. 
    \item Recent success shows the success of visuomotor imitation learning (robomimic bekerley paper) by directly using behavior cloning
    \item While behavior cloning has shown its outstanding performance in robot manipulation, a long-standing issue: generalize poorly to variations. This is because the end-to-end visuomotor imitation learning only learns the spurious correlation between pixels and actions. 
    \item We propose our approach OCIL
    
    \item Our contribution: 1) An imitation learning approach that is based on task-agnostic object-centric representation; 2) TBD; 3) We demonstrate the effectiveness of the proposed imitation learning both in simulation and on real robots.
\end{itemize}




(old notes):
\begin{itemize}
    \item Real-world manipulation tasks are challenging.
    \item Imitation learning has been a data-efficient paradigm for robots to learn a policy without hand-designing motor programs.
    \item There have been successful cases to demonstrate imitation learning for visuomotor control.
    \item Yet existing approaches fall short in systematic generalization: when a robot encounters sensory readings that are out-of-distribution, the learned policies learned significantly. This pitfall stands out even more when we use image observations. This is because vanilla behavior cloning only learns spurious correlations between pixels and actions, thus failing to generalize to observations where object placements are not in the training distribution. )
    \item There are several ways to improve the generalization. 1) Add data augmentation techniques to artificially increase the variations of demonstration dataset, and that can increase the systematic generalization; 2) 
    Interactive approaches that either query human or regularization base approaches. (such as Dagger, GAIL). State the limitations of both works.
    \item We provide another aspect to increase the systematic generalization (we might want to explain what is systematic generalization first) of imitation learning in robot manipulation tasks. The key insight is that a major focus of contact-rich robot manipulation tasks is to manipulate objects. Thus, understanding "objectness" from sensory observations becomes crucial. By injecting this inductive bias, we hope to see that the imitation learning policy first discover the relation between the pixel-level percepts and "objects", then correlate "object" observations with actions. In this way, we bypass the issue for robots to learn spurious correlation between the pixel-level obsearvations and actions.
    % So the inductive bias of objects are natural and essential way to achieve data-efficient, robust imitation learning policies. We would like to learn an imitation learning policy for a robot manipulation tasks using the same amount of demonstration data as in the existing visuomotor imitation learning literature, without having additional annotations of objects in the perception.
\end{itemize}




==> experiment_writeup.tex <==
% Here I write down all the approach details

\section{Experiment}
\subsection{Environment designs}
We design three 

\subsection{Simulation + real-world details}


To evaluate the robustness of our models, we design three additional task variants for each environment. (Cite systematic generalization paper). 

\subsection{Experiment/model parameters and details}

For baseline models such as BC and BC-RNN, we used the hyperparameters from Mandlekar et al.~\cite{} for comparison. In order to avoid showing inflated performance of models~\cite{} (sergey's offline paper), we obtain the model that has the least loss after all training for all environments.

Aside from presenting our results in the main text, we also include additional evaluation in the appendix to show that our comparison result is consistent in tasks from robomimic~\cite{}.

\subsection{Evaluation details}
\paragraph{}

\paragraph{Consistent initialization evaluation} We observed that the task performance of each model varies a lot in simulation because of the randomness of initialization, and in order to obtain apple-to-apple comparison, we propose the following evaluation setup: we generate $200$ randomly initialized scenes for each evaluation, and compute the mean performance of the task. In this way, we can directly see the task performance differences.

For real robot experiments, because it's hard to achieve the exact same initialization setup as we can in simulation, we randomly place the objects in the scene and try to replicate the visually similar scenes for the evaluation. For each round of evaluation, we evaluate every model three times so that we can get consistent and robust evaluation. 


\subsection{Results analysis}


